Parameter Expanded Stochastic Gradient Markov Chain Monte Carlo

Bayesian Neural Networks (BNNs) provide a promising framework for modeling predictive uncertainty and enhancing out-of-distribution robustness (OOD) by estimating the posterior distribution of network parameters. Stochastic Gradient Markov Chain Monte Carlo (SGMCMC) is one of the most powerful methods for scalable posterior sampling in BNNs, achieving efficiency by combining stochastic gradient descent with second-order Langevin dynamics. However, SGMCMC often suffers from limited sample diversity in practice, which affects uncertainty estimation and model performance. We propose a simple yet effective approach to enhance sample diversity in SGMCMC without the need for tempering or running multiple chains. Our approach reparameterizes the neural network by decomposing each of its weight matrices into a product of matrices, resulting in a sampling trajectory that better explores the target parameter space. This approach produces a more diverse set of samples, allowing faster mixing within the same computational budget. Notably, our sampler achieves these improvements without increasing the inference cost compared to the standard SGMCMC. Extensive experiments on image classification tasks, including OOD robustness, diversity, loss surface analyses, and a comparative study with Hamiltonian Monte Carlo, demonstrate the superiority of the proposed approach.

==> main/_deprecated_background.tex <==
\section{Preliminaries}
\label{sec:main:background}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notation}

We begin by presenting the mathematical formulation of neural networks.
Specifically, a fully connected feed-forward neural network with $L$ layers transforms maps $\bsx=\bsh^{(0)}$ to outputs $\bsy=\bsh^{(L)}$ through the following transformations:
% \[\label{eq:mlp}
% \bsh^{(l)} = \sigma(\bW^{(l)}\bsh^{(l-1)} + \bsb^{(l)}), \text{ for } l=1,\dots,L-1, \text{ and }
% \bsh^{(L)} = \bW^{(L)}\bsh^{(L-1)} + \bsb^{(L)},
% \]
\[\label{eq:mlp}
\bsh^{(l)} = \sigma(\bW^{(l)}\bsh^{(l-1)}), \text{ for } l=1,\dots,L-1, \text{ and }
\bsh^{(L)} = \bW^{(L)}\bsh^{(L-1)},
\]
where $\bsh^{(l)}$ denotes the feature at the $l^\text{th}$ layer, $\bW^{(l)}$ represents the weight parameters at the $l^\text{th}$ layer, and $\sigma(\cdot)$ indicates the activation function.
While we have omitted the bias term for simplicity, our practical implementations do include it.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Permutation Invariance of Neural Networks}

% For any $L$-layered ($L>1$) architecture with the nonlinearities such as ReLU and SWISH, which are element-wise independent operation, their weight matrices always have the permutation invariance along the channel-wise dimensions (the kernel dimension in the convolution layers does not element-wise independent).

% \textbf{Notation.}
% We begin by presenting the mathematical formulation of neural networks.
% Specifically, a fully connected feed-forward neural network with $L$ layers transforms maps $\bsx=\bsh^{(0)}$ to outputs $\bsy=\bsh^{(L)}$ through the following transformations:
% \[\label{eq:mlp}
% \bsh^{(l)} = \sigma(\bW^{(l)}\bsh^{(l-1)} + \bsb^{(l)}), \text{ for } l=1,\dots,L-1, \text{ and }
% \bsh^{(L)} = \bW^{(L)}\bsh^{(L-1)} + \bsb^{(L)},
% \]
% where $\bsh^{(l)}$ denotes the feature at the $l^\text{th}$ layer, $\bW^{(l)}$ and $\bsb^{(l)}$ respectively are the weight and bias parameters at the $l^\text{th}$ layer, and $\sigma(\cdot)$ represents the nonlinearity.
% Here, we use element-wise independent functions such as ReLU~\citep{fukushima1969visual,nair2010rectified} and Swish~\citep{hendrycks2016gaussian,elfwing2018sigmoid,ramachandran2017searching} for the nonlinearity to ensure the permutation invariance along the channel-wise dimensions.
% Note that this permutation invariance does not apply to the kernel dimensions in convolutional layers, where the operations are not element-wise independent.

% \textbf{Permutation invariance.}
% In \cref{eq:mlp}, reordering the intermediate nodes, which is equivalent to multiplying a permutation matrix on both the left and right sides of the nonlinearity, yields an equivalent function, thus the permutation invariance holds.
% More precisely, for any permutation matrix $\bP$ and element-wise independent operation $\sigma$ such as ReLU~\citep{fukushima1969visual,nair2010rectified} and Swish~\citep{hendrycks2016gaussian,elfwing2018sigmoid,ramachandran2017searching}, we can derive the following for the $l^\text{th}$ layer,
% \[
% \sigma(\bW^{(l)} \bsh^{(l-1)} + \bsb^{(l)}) = \bP\tr \sigma(\bP \bW^{(l)} \bsh^{(l-1)} + \bP \bsb^{(l)})
% \]
% from the fact that $\bP\tr\bP = \bI$ and $\sigma(\cdot) = \bP\tr\bP\sigma(\cdot) = \bP\tr\sigma(\bP\cdot)$.
% Moreover, permutation in one layer can be seen as affecting the weight in the subsequent layer.
% Specifically, when permutation matrices $\bP\lyr{l-1}$ and $\bP\lyr{l}$ respectively are introduced for the $(l-1)^\text{th}$ and $l^\text{th}$ layers, i.e.,
% \[
% \bP\lyrt{l} \sigma(
%     {\color{blue} \bP\lyr{l} \bW\lyr{l} \bP\lyrt{l-1}} \sigma(
%         % \cdots
%         \bP\lyr{l-1}\bW\lyr{l-1}\bsh\lyr{l-2} + \bP\lyr{l-1}\bsb\lyr{l-1}
%     ) + {\color{blue}\bP\lyr{l}\bsb\lyr{l}}),
% \]
% the weight of the $l^\text{th}$ layer is enveloped by two permutation matrices, while the bias is influenced by only one (highlighted in blue).
% Consequently, we define the \textit{permuted parameters} for the weight and bias parameters at the $l^\text{th}$ layer as follows:
% \[
% \pi(\bW\lyr{l}) = \bP\lyr{l}\bW\lyr{l}\bP\lyrt{l-1}, \quad
% \pi(\bsb\lyr{l}) = \bP\lyr{l}\bsb\lyr{l},
% \]
% where $\bP\lyr{0} = \bP\lyr{L} = \bI$, since reordering the input or output is not invariant.
% While we illustrate the permutation invariance using a fully connected feed-forward neural network, the same approach can be extended to other structures, including residual connections and convolutional layers.

% For any $L$-layered ($L>1$) architecture with the nonlinearities such as ReLU~\citep{fukushima1969visual,nair2010rectified} and Swish~\citep{hendrycks2016gaussian,elfwing2018sigmoid,ramachandran2017searching}, which are element-wise operations, the weight matrices exhibit permutation invariance along the channel-wise dimensions\footnote{Note that this permutation invariance does not apply to the kernel dimensions in convolutional layers, where the operations are not element-wise independent.}.
% For example, consider an $L$-layered multi-layer perceptron (MLP) that maps inputs $\bsx = \bsh\lyr{0}$ to outputs $\bsy = \bsh\lyr{L}$,
% \[
% \bsh\lyr{l} = \sigma(\theta\lyr{l}\bsh\lyr{l-1}+\eta\lyr{l}), \text{ for } l=1,\dots,L-1, \text{ and }
% \bsh\lyr{L} = \theta\lyr{L}\bsh\lyr{L-1}+\eta\lyr{L},
% \]
% where $\theta\lyr{l}$ and $\eta\lyr{l}$ respectively are the weight and bias parameters at the $l^\text{th}$ layer, $\sigma(\cdot)$ denotes the nonlinearity, and $\bsh\lyr{l}$ denotes the feature at the $l^\text{th}$ layer.
% Reordering the intermediate nodes corresponds to multiplying a permutation matrix on left and right sides of the nonlinearity and it produces an equivalent function, thereby the following invariance holds:
% \[
% \label{eq:invariance}
% \sigma(\theta\lyr{l}\bsh\lyr{l-1}+\eta\lyr{l})=P\tr\sigma(P\theta\lyr{l}\bsh\lyr{l-1}+P\eta\lyr{l}),\quad \forall P\in\calS,
% \] where $P$ is a permutation matrix. \cref{eq:invariance} can be derived from the fact that $P\tr P = I$ and the nonlinearity $\sigma$ is element-wise independent operation:
% \[
% \sigma(\cdot)=P\tr P\sigma(\cdot)=P\tr\sigma(P\cdot).
% \]
% For the $l$-th and $l+1$-th layer, the weight parameter is enveloped by two different $P$:
% \[
% \theta\lyr{l+1}P\lyrt{l}\sigma(P\lyr{l}\theta\lyr{l}P\lyrt{l-1}\bsh\lyr{l-1}+P\lyr{l}\eta\lyr{l}) + \eta\lyr{l+1}.
% \]
% Consequently, the permuted parameters $\pi(\theta\lyr{l})$ and $\pi(\eta\lyr{l})$ can be described as
% \[
% \pi(\theta\lyr{l}) &= P\lyr{l}\theta\lyr{l}P\lyrt{l-1}, & \pi(\eta\lyr{l}) &= P\lyr{l}\eta\lyr{l},
% \] for $l=2,3,\ldots,L-1$. For $l=1$ and $L$, $\pi(\theta^{(1)})=P^{(1)}\theta^{(1)}$ and $\pi(\theta\lyr{l})=\theta\lyr{l} P\lyrt{l-1}$, respectively, because reordering input or output is not invariant.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bayesian Inference with Stochastic Gradient MCMC}

\textbf{Bayesian model averaging.}
In Bayesian inference, our goal is not to find a single best estimate of the parameters, such as the maximum a posteriori estimate, but instead to sample from the posterior distribution $p(\btheta | \calD)$ of the parameters $\btheta$ given the observed data $\calD$.
The prediction for a new datapoint $x$ is then given by Bayesian model averaging (BMA),
\[\label{eq:bma}
p(y | x, \calD) = \int p(y | x, \btheta) p(\btheta | \calD) \dee\btheta,
\]
which can be approximated by Monte Carlo integration $p(y|x,\calD) \approx \sum_{m=1}^{M} p(y|x,\btheta_{m}) / M$ using finite posterior samples $\btheta_{1}, \dots, \btheta_{M} \sim p(\btheta | \calD)$.
In Bayesian deep learning, we typically introduce several sampling methods to obtain the posterior samples, as the posterior distribution of the neural network parameters $\btheta$ cannot be expressed in closed form in practice.

\textbf{Stochastic Gradient MCMC.}
Hamiltonian Monte Carlo~\citep[HMC;][]{duane1987hybrid,neal2012mcmc} is the gold standard sampling method that asymptotically generates samples from the posterior distribution.
Defining the negative of the unnormalized log-posterior as the \textit{potential energy},
\[
U(\btheta) = -\log{p(\calD | \btheta)} - \log{p(\btheta)},
\]
HMC obtains a sequence of posterior samples by simulating Hamiltonian dynamics targeting the posterior distribution $p(\btheta | \calD)$.
However, it requires computing the gradient $\nabla_\btheta U(\btheta)$ over the entire dataset $\calD$, which becomes intractable for large-scale datasets.
To resolve this, Stochastic Gradient Hamiltonian Monte Carlo~\citep[SGHMC;][]{chen2014stochastic} introduce a noisy estimate of the energy,
\[
\tilde{U}(\btheta) = -\frac{|\calD|}{|\calB|}\log{p(\calB | \btheta)} - \log{p(\btheta)},
\]
where the log-likelihood is computed only for a mini-batch of data $\calB \subset \calD$, and the full-data gradient is replaced by the mini-batch gradient.
By introducing additional friction and Gaussian noise terms along with the decaying series of step sizes, SGHMC ensures the convergence to the same stationary distribution as the original HMC.
As a result, an SGHMC update step is given as follows:
\[
\btheta &\gets \btheta + \epsilon \bM^{-1} \bsr \\
\bsr &\gets (1 - \epsilon \bC \bM^{-1}) \bsr - \epsilon \nabla_{\theta}\tilde{U}(\btheta) + \calN(0, 2(\bC - \hat{\bB}) \epsilon),
\]
where $\bsr$ is the momentum, $\epsilon$ is the step size, $\bM$ is the mass matrix, $\bC$ is the friction term, and $\hat{\bB}$ corrects for the stochastic gradient noise.
% Since SGHMC is one of the most powerful Stochastic Gradient Markov Chain Monte Carlo (SGMCMC) methods, with its Markov chain simulated as second-order Langevin dynamics, we will use SGHMC as a representative of SGMCMC in this paper.


% Following common practice~\citep{zhang2020cyclical,izmailov2021bayesian}, $\hat{\bB}$ is set to zero, $\bM$ is chosen as the identity matrix, and a cyclical schedule is employed for the step sizes in our experiments.



% In Bayesian deep learning, our goal is to estimate the posterior distribution of the neural network parameters $\theta$ given a dataset $\calD$, denoted as $p(\theta|\calD)$.
% However, due to the intractability of the posterior distribution, we often work with its unnormalized form $p(\calD|\theta)p(\theta)$, which is proportional to the posterior $p(\theta|\calD)$.
% In particular, HMC constructs the potential energy as:
% \[
% U(\theta) = -\log p(\calD|\theta) -\log p(\theta),
% \]
% and simulates Hamiltonian dynamics based on this potential energy.
% For classification tasks, the first term typically corresponds to the cross-entropy loss, while the second term represents $\ell_{2}$-norm regularization of $\theta$.

% On the other hand, SGMCMC is designed to take account the computional efficiency and utility of stochastic gradients induced from the mini-batch. It estimates the log-likelihood as
% \[
% \tilde{U}(\theta) = -\frac{|\calD|}{|\calB|}\log p(\calB|\theta) - \log p(\theta),
% \] where $\calB$ is a mini-batch taken from $\calD$ and additionally schedules the step size asymptotically going to zero to eliminate the Metropolis-Hastings (MH) step in HMC. Stochastic Gradient Hamiltonian Monte Carlo (SGHMC)~\citep{chen2014stochastic} is one of the powerful SGMCMC method that its Markov chain is simulated as the second order Langevin dynamics~\citep{wang1945on}. To reduce the error occurred from the stochastic gradients, SGHMC adopts extra friction and Gaussian noise in the simulation. As a result, one step of SGHMC is defined as follows:
% \[
% \theta &\leftarrow \theta + \epsilon_t M^{-1} r\\
% r &\leftarrow (1-\epsilon_t CM^{-1})r - \epsilon_t\nabla\tilde{U}(\theta) + \calN(0, 2(C-\widehat{B})\epsilon_t),
% \] where $\epsilon_t$ is the step size, $r$ is momentum, $M$ is the mass of the momentum distribution, $C$ is the magnitude of friction, $\widehat{B}$ is the correction for the stochastic gradient error. In our experiments, we use the cyclical step size \citep{zhang2020cyclical}, which schedule $\epsilon_t$ to be periodically increased and decreased. Additionally, we set the correction $\widehat{B}$ zero, the setting widely used in the practical SGMCMC scenarios \red{[citations]}.

% We can regard the samples $\{\theta_i\}_{i=1}^K$ are approximately drawn from the posterior $p(\theta|\calD)$. In the inference step, we average the outputs of models determined by the collected $\theta$ samples:
% \[
% p(\bsy|\bsx,\calD)=\int p(\bsy|\bsx,\theta)p(\theta|\calD)\dee\theta \approx \sum_{i=1}^K p(\bsy|\bsx,\theta_i)
% \] where $p(\bsy|\bsx, \theta)$ is the distribution of model outputs such as the confidence probabilities of classifiers. The more diverse the samples $\theta_i$ are collected, the more accurate the posterior is estimated. Due to this reason, several prior works have suggested methods to improve the diversity but they are still limited to reach the diversity of DE \red{[citations]}.

==> main/_deprecated_introduction.tex <==
\section{Introduction}
\label{sec:main:introduction}

Bayesian deep learning or Bayesian Neural Network (BNN) has raised an importance of model calibration in terms of out-of-distribution robustness  \red{[citations]}. Unlike regular training of neural networks (NNs), BNN requires to estimate the posterior distribution $p(\theta|\calD)$, where $\theta$ is the BNN parameters and $\calD$ is the given dataset. There are variational~\citep{liu2016stein,blei2017variational} and sampling approaches to estimate the posterior and one of the representative sampling method is stochastic gradient Markov chain Monte Carlo~\citep[SGMCMC;][]{welling2011bayesian,chen2014stochastic,ma2015complete}. SGMCMC has showed great success in the large scale Bayesian inference regime by leveraging both the exploitation of stochastic gradient descent (SGD) and the exploration of Hamiltonian Monte Carlo~\citep[HMC;][]{duane1987hybrid}. It is a stochastic differential equation that approximately draw samples from the posterior. Since $p(\theta|\calD)$ is intractable, the algorithm instead compute its unnormalized distribution, $p(\calD|\theta)p(\theta)$, during sampling. In classification task, $p(\calD|\theta)$ is often described as products of the categorical distribution where each probabilities are the confidence of NN $\theta$ and we set $p(\theta)$ the isotropic Gaussian distribution.

Despite of its powerful performance, SGMCMC suffers from weak diversity across the samples compared to another method called deep ensemble~\citep[DE;][]{lakshminarayanan2017simple}. The samples of DE are collected by SGD training of a single NN with different random initializations. DE is technically not a BNN method but it ends up with good performance of BNN with high diversity of samples, which leads to better uncertainty estimation and model calibration~\citep{ovadia2019can,ashukha2020pitfalls}. Once the budget of training time is not limited, DE mostly outperform SGMCMC in terms of both accuracy and uncertainty estimation. Moreover, the MCMC methods including SGMCMC chronically have suffered from sampling multi-modal distributions due to strong correlation between the current and previous samples as Markov chains.

\red{[Efforts of prior works to overcome the diversity issues]}

In this paper, we resolve that issue by utilizing the symmetry information intrically possessed in the NNs, permutation invariance. NNs can be regarded as a graph whose edges are learnable parameters. The thing is even if we exchange two hidden nodes in the same layer, which equivalent to the exchange the both columns of the next weight and rows of the previous weights, the output of an $L$-layered Multilayer percerptron (MLP) $f$ does not change as follows:
\[
&f(\theta\lyr{1},\ldots,\theta\lyr{l}, \eta\lyr{1},\ldots,\eta\lyr{l})= f(\pi(\theta\lyr{1}),\ldots,\pi(\theta\lyr{l}),\pi(\eta\lyr{1}),\ldots,\pi(\eta\lyr{l})),\\
&\pi(\theta\lyr{l}) = P\lyr{l}\theta\lyr{l}P\lyrt{l-1},\quad\quad \pi(\eta\lyr{l}) = P\lyr{l}\eta\lyr{l},
\] where $\theta\lyr{l}\in \bbR^{n_l\times n_{l-1}}$ and $\eta\lyr{l}\in \bbR^{n_l}$ are the weight and bias parameters at layer $(l)$, $P\lyr{l}\in\{0,1\}^{n_l\times n_l}$ and $P\lyr{l-1}\in\{0,1\}^{n_{l-1}\times n_{l-1}}$ are permutation matrices reordering $l$-th layer and $l-1$-th layer, respectively.
By applying random permutation on a SGMCMC sample, we can get an equivalent but extremely far sample. Basically, a short SGMCMC trajectories are often limited in a single basin consisting of local modes exhibiting less diversity. If we can approximately permute the solution but not exactly, the transitioned solution will be far away from the original solution but not equivalently as the exact permutation. i.e. we take exploration from the permutation-like transition, which leads to diversity due to the broken permutation.

Inspired from this intuition, we propose a novel SGMCMC method that augment a new parameter $Q$ being in charge of exploration as permutation. $Q$ is applied into the parameters of NNs as the same structure as permutation matrices according to the invariance. However, $Q$ is not constrained in the permutation space and rather flows on Euclidean space through the SGMCMC dynamics. In the end, $Q$ enjoys the structure of permutation operations but naturally avoid the exact permutation, which hinders sample diversity of SGMCMC. In other words, the weight and bias parameters in the intermediate linear layer of a MLP as follows:
\[
\phi\lyr{l} &= Q\lyr{l}\theta\lyr{l}Q\lyrt{l-1}, & \xi\lyr{l} &= Q\lyr{l}\eta\lyr{l},
\] where $Q\lyr{l}\in\bbR^{n_l\times n_l}$ and $Q\lyr{l-1}\in\bbR^{n_{l-1}\times n_{l-1}}$ are augmented parameters multiplied in each layer. Note that $Q$ is sampled from usual SGMCMC algorithms as $\theta$ and $\eta$.

\red{[Why does $Q$ work?!?!?!]}

==> main/_deprecated_method.tex <==
\section{Deep Linear Reparametrization}
\label{sec:main:method}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reparametrization}

The diversity of samples itself is roughly easy to achievable if we just increase the step size large enough and let SGMCMC explores to a suboptimal posterior distribution. In that case, however, the mixing time or convergence rate towards the target posterior is extremely slow, thereby the BMA performance is not guaranteed for a given training budget. Thus, we focus on the convergence rate instead of directly diversifying the SGMCMC dynamics.

The depth of a neural network is one of the key factor to increase the performance of gradient descent (GD) or SGD in deep learning. A trained deeper neural network often outperforms a shallow network in both convergence and generalization \citep{sun2016on,hayou2022exact}. This statement similarly holds for deep linear neural networks (DLNNs) under some assumptions on the weight matrices \citep{arora2019convergence,he2024information}. Although the multiplication of every weight matrices in DLNN is equivalent to a single layer, which leads to the same expressive power in the inference, their gradient descents differ from that of DLNN and the difference induces the fast convergence of DLNN. We can also notice that their inference costs are identical.

Based on those advantages, we reparametrize a given $L$-layer MLP $f$ whose parameter is $\btheta=(\bW\lyr{1},\bW\lyr{2},\ldots,\bW\lyr{L})$ in \cref{eq:mlp} as
\[
\label{eq:reparametrization}
&\bW\lyr{l} = \bP_{1:c}\lyr{l}\bV\lyr{l}\bQ_{1:d}\lyr{l},\quad\text{and}\quad\bb\lyr{l}=\bP_{1:d}\lyr{l}\ba\lyr{l},\quad\text{for }l=1,2,\ldots,L,\nonumber \\
&\bP_{1:c}\lyr{l} = \bP_{c}\lyr{l}\cdots\bP_2\lyr{l}\bP_1\lyr{l}\quad\text{and}\quad \bQ_{1:d}\lyr{l} = \bQ_1\lyr{l}\bQ_2\lyr{l}\cdots\bQ_{d}\lyr{l},
\] where $\bV\lyr{l}\in\bbR^{n_l\times n_{l-1}}$ is a base weight matrix, $\bP_i\lyr{l}\in\bbR^{n_l \times n_l}$, $\bQ_i\lyr{l}\in\bbR^{n_{l-1} \times n_{l-1}}$ are the expanded matrices, and $e=c+d\geq 0$ is the number of the expanded matrices. We call this \emph{expanded parametrization} (EP) $e=0$ denotes the standard parameterization (SP). Note that although $\bP_i\lyr{l}$ and $\bQ_i\lyr{l}$ are not necessary to be square matrices, their multiplication $\bP_{1:c}\lyr{l}$ and $\bQ_{1:d}\lyr{l}$ must be square matrices to maintain the dimension of $\bW$ when $\bV$ holds the dimension of $\bW$. Nonetheless, we set $\bP_i\lyr{l}$ and $\bQ_i\lyr{l}$ also square in order to save memory cost while preserving convergence stability of $\bP_{1:c}\lyr{l}$ and $\bQ_{1:d}\lyr{l}$, only guaranteed when the width of intermediate dimension of DLNN should be greater and equal to both input and output dimensions \citep{laurent2018deep,du2019width}.

\red{[The example SGHMC dynamics for the new parametrization]}

\begin{thm} 
Consider SGLD with EP, $\bP_{1:c}\lyr{l}\bV\lyr{l}\bQ_{1:d}\lyr{l}$, corresponding to \cref{eq:reparametrization} and assume that the initialization of the parameters follows Theorem 1 in \citet{arora2018on} and the SGLD follows Assumption 1 and Assumption 2 in \citet{chen2015on} for $k\leq 1$. Then, compared to the SP, $\bV\lyr{l}$, with the same step size, the convergence rate of EP is $\sigma_\text{min}(\bP_{1:c}\lyr{l}\bV\lyr{l}\bQ_{1:d}\lyr{l})^{2(c+d)/(c+d+1)}$ times faster and the bound of the distance between the samples is $\norm{\overline{\bP}}_2^L$ times larger, where $\sigma_\text{min}(\bM)$ denotes the minimum eigenvalue of the matrix $\bM$ and $\norm{\overline{\bP}}_2$ is the operator 2-norm of a bound of $\bP_{1:c}\lyr{l}$ or $\bQ_{1:d}\lyr{l}$. i.e. EP has better exploitation and exploration.
\end{thm}

\begin{proof}
    The proof consists of the convergence analysis and the sample distance comparison. As the extension of the SGLD convergence analysis \citep{chen2015on}, we applied the gradient updates of the multiplied value $\bP\bV\bQ$ which differs from that of single matrix $\bV$ as described in the implicit acceleration of DLNN \citep{arora2018on}.

    By Theorem 1 and Claim 1 in~\citet{arora2018on}, the dynamics of the multiplied parameter with vectorization $\bX=\V{\bW}$ for $\bW\lyr{l} = \bP_{1:c}\lyr{l}\bV\lyr{l}\bQ_{1:d}\lyr{l}$ is as follows:
    \[
    \dee\bX(t) = - P_{\bX(t)}\nabla\calF(\bX(t)),
    \] where $\V{\bM}$ stands for vectorization of the matrix $\bM$, $\calF$ is an arbitrary function that determines the dynamics of $\bX(t)$, and $P_{\bX(t)}$ is a positive semidefinite matrix whose eigenvalues are greater than or equal to $\sigma_\text{min}(\bW(t))^{2(c+d)/(c+d+1)}$. Applying to the SGLD dynamics, the diffusion of EP can be described as:
    \[
    \dee\bX(t) = - P_{\bX(t)}\nabla\tilde{U}(\bX(t))\dee t + B\dee W_t,
    \] where $W$ is Brownian motion and the $B$ is the standard deviation of the diffusion noise.

    According to \citet{chen2015on}, the difference between the samples and the target can be expanded as
    \[
    \hat{\phi}-\overline{\phi} &= \frac{\bbE[\phi(\bX(T))]-\phi(\bX(0))}{S_T} + \frac{1}{S_T}\sum_{t=1}^{T-1}\left(\bbE[\psi(\bX(t-1))]-\psi(\bW(t-1))\right) \\& - \sum_{t=1}^{T}\frac{\epsilon_t}{S_T}\Delta \calV_t\psi(\bW(t-1)) - C\frac{\sum_{t=1}^T\epsilon_t^2}{S_T},
    \] where $T$ is the number of samples, $S_T=\sum_{t=1}^T \epsilon_t$ and $\calV_t=P_\bX(t)(\nabla\tilde{U}_t-\nabla U)\cdot\nabla_\bX$. Since the eigenvalues of $P_{\bX(t)}$ are greater than or equal to $\sigma_\text{min}$
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Prior Distributions}

The new parametrization should improve the functional diversity of the given neural network, while its gradients should neither vanish nor explode. To enhance functional diversity while preserving the inference cost, we adopt an expanded linear layer as follows:
\[
 A\lyr{l} \theta\lyr{l} B\lyr{l-1} \bsh\lyr{l-1} + A\lyr{l} \eta\lyr{l},
\]
where $A \in \bbR^{n_l \times n_l}$ and $B \in \bbR^{n_{l-1} \times n_{l-1}}$ are square matrices learned along with $\theta$ and $\eta$. In the inference procedure, we can merge $\phi\lyr{l} = A\lyr{l} \theta\lyr{l} B\lyr{l}$ and $\xi\lyr{l} = A\lyr{l} \eta\lyr{l}$, and treat it as an ordinary linear layer, which conserves the inference costs. For a two-layer MLP, we can describe it as:
\[
\label{eq:expanded-mlp}
A\lyr{l+1} \theta\lyr{l+1} B\lyr{l} \sigma \left( A\lyr{l} \theta\lyr{l} B\lyr{l-1} \bsh\lyr{l-1} + A\lyr{l} \eta\lyr{l} \right) + A\lyr{l+1} \eta\lyr{l+1},
\]
where $\sigma$ is a nonlinearity function whose gradient is bounded. Compared to the ordinary MLP,
\[
\label{eq:ordinary-mlp}
\theta\lyr{l+1} \sigma \left( \theta\lyr{l} \bsh\lyr{l-1} + \eta\lyr{l} \right) + \eta\lyr{l+1},
\]
the new MLP could fluctuate significantly due to maximizing the Lipschitz continuity via $A$ and $B$ without constraints. Therefore, we need to impose some constraints by either modifying their structure or defining a prior distribution for $A$ and $B$.

\begin{thm}
For an MLP with the expanded linear layer as in \cref{eq:expanded-mlp}, the matrices $A\lyr{l}$ and $B\lyr{l}$ that conserve both the gradient bound and the Lipschitz constant, same as the ordinary MLP, are scaled orthogonal matrices. Specifically, they must take the form $A\lyr{l} = \alpha Q$ and $B\lyr{l} = Q\tr / \alpha$, where $Q$ is an orthogonal matrix, i.e., $Q\tr Q = QQ\tr = I$, and $\alpha \in \bbR$ is a scalar.
\end{thm}

\begin{proof}
Consider \cref{eq:expanded-mlp} as an MLP with a modified nonlinearity $\tilde{\sigma}(\cdot) = B \sigma (A \cdot)$, where $A$ and $B$ are the weight matrices. Thus, we compare this form with the ordinary MLP in terms of the Lipschitz constant and gradient bounds.

Let $\sigma$ be a nonlinearity with a derivative bounded by a constant $G > 0$, i.e., $\forall z \in \bbR$, 
\[
\norm{\sigma'(z)}_2 \leq G,\quad\text{or equivalently}\quad \forall \bsz \in \bbR^n, \quad \abs{\frac{\partial \sigma(\bsz)_i}{\partial \bsz_i}} \leq G, \quad \text{and } \abs{\frac{\partial \sigma(\bsz)_i}{\partial \bsz_j}}_{i \neq j} = 0.
\]
The derivative of the modified nonlinearity $\tilde{\sigma}(\bsz) = B \sigma (A \bsz)$ is bounded as:
\[
\abs{\frac{\partial (B \sigma(A \bsz))_i}{\partial \bsz_j}} = \abs{ \left( B \diag (\sigma'(A \bsz)) A \right)_{ij}} \leq G \abs{(BA)_{ij}}.
\]
The inequality holds by Cauchy-Schwarz inequality in the element-wise expression. For the gradient bound to be preserved, we require $\abs{(BA)_{ij}} = 1$ when $i = j$ and $\abs{(BA)_{ij}} = 0$ when $i \neq j$. This condition implies $BA = \pm I$, or equivalently, $B = \pm A^{-1}$.

Next, let $\sigma$ be $L$-Lipschitz continuous, i.e., $\forall \bsz_1, \bsz_2 \in \bbR^n$, 
\[
\norm{\sigma(\bsz_1) - \sigma(\bsz_2)}_2 \leq L \norm{\bsz_1 - \bsz_2}_2.
\]
The Lipschitz constant of the modified nonlinearity $\tilde{\sigma}$ is bounded by the operator norm inequality:
\[
\norm{B \sigma(A \bsz_1) - B \sigma(A \bsz_2)}_2 \leq L \norm{B}_2 \norm{A}_2 \norm{\bsz_1 - \bsz_2}_2,
\]
where $\norm{A}_2$ and $\norm{B}_2$ are the operator norms of $A$ and $B$, respectively. To preserve the Lipschitz continuity, we must have $\norm{B}_2 \norm{A}_2 = 1$. Given $B = \pm A^{-1}$, we have $\norm{A}_2 \norm{A^{-1}}_2 = 1$. 

Since the operator norm corresponds to the largest singular value, we express this as:
\[
\norm{A}_2 = \lambda_1, \quad \norm{A^{-1}}_2 = 1/\lambda_n,
\]
where $\lambda_1$ and $\lambda_n$ are the largest and smallest singular values of $A$, respectively. Their product being 1 implies:
\[
\lambda_1 / \lambda_n = 1, \quad \text{or equivalently } \lambda_1 = \lambda_n.
\]
Thus, all singular values of $A$ must be equal, meaning $A$ is a scaled orthogonal matrix, i.e., $A = \alpha Q$, where $\alpha \in \bbR$ is a scalar and $Q$ is an orthogonal matrix, i.e., $Q\tr Q = I$. Since $B = \pm A^{-1}$, we conclude that $B = Q\tr / \alpha$.
\end{proof}

Just for reference:

Provable Benefit of Orthogonal Initialization in Optimizing Deep Linear Networks \citep{hu2020provable}

Scaled Orthogonal Gaussian Distribution:
\[
p(Q) \propto \exp\left(-\frac{\norm{Q\tr Q-\alpha I}^2+\norm{QQ\tr - \alpha I}^2}{4\sigma^2}\right),
\] where $\alpha$ is the scaling factor.

\subsection{Relationship to Riemannian Manifold LD and Preconditioned SGLD}
There is relationship only in langevin dynamics as a precondition matrix.

==> main/_deprecated_method_exploitation.tex <==
\section{Quick SGMCMC}
\label{sec:main:method}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reparametrization}

The diversity of samples itself is roughly easy to achievable if we just increase the step size large enough and let SGMCMC explores to a suboptimal posterior distribution. In that case, however, the mixing time or convergence rate towards the target posterior is extremely slow, thereby the BMA performance is not guaranteed for a given training budget. Thus, we focus on the convergence rate instead of directly diversifying the SGMCMC dynamics.

The depth of a neural network is one of the key factor to increase the performance of gradient descent (GD) or SGD in deep learning. A trained deeper neural network often outperforms a shallow network in both convergence and generalization \citep{sun2016on,hayou2022exact}. This statement similarly holds for deep linear neural networks (DLNNs) under some assumptions on the weight matrices \citep{arora2019convergence,he2024information}. Although the multiplication of every weight matrices in DLNN is equivalent to a single layer, which leads to the same expressive power in the inference, their gradient descents differ from that of DLNN and the difference induces the fast convergence of DLNN. We can also notice that their inference costs are identical.

{\color{blue}
We introduce the \textit{expanded parametrization} (EP) of an $L$-layer MLP, defined in \cref{eq:mlp}, with parameters $\btheta = (\bW\lyr{1},\dots,\bW\lyr{L}, \bsb\lyr{1},\dots,\bsb\lyr{L})$ as
\[\label{eq:reparametrization}
\bW\lyr{l} = \bP_{1:c}\lyr{l} \bV\lyr{l} \bQ_{1:d}\lyr{l}
\text{ and } \bsb\lyr{l} = \bP_{1:c} \bsa\lyr{l}, \text{ for } l=1,\dots,L,
\]
where $\bP_{1:c}\lyr{l} \triangleq \bP_{c}\lyr{l} \cdots \bP_{1}\lyr{l}$ and $\bQ_{1:d}\lyr{l} \triangleq \bQ_{1}\lyr{l} \cdots \bQ_{d}\lyr{l}$.
While the \textit{expanded matrices} $\bP_{i}\lyr{l}$ and $\bQ_{i}\lyr{l}$ do not need to be square, their multiplications, $\bP_{1:c}\lyr{l}$ and $\bQ_{1:d}\lyr{l}$, must be square to ensure that the \textit{base matrix} $\bV\lyr{l}$ retains the same dimensionality as $\bW$.
Meanwhile, we also set the expanded matrices $\bP_{i}\lyr{l}$ and $\bQ_{i}\lyr{l}$ to be square to reduce memory costs while preserving the convergence stability of their multiplications $\bP_{1:c}\lyr{l}$ and $\bQ_{1:d}\lyr{l}$, which is guaranteed only when the width of intermediate dimensions in the DLNN is greater than or equal to both the input and output dimensions~\citep{laurent2018deep,du2019width}.
}

Based on those advantages, we reparametrize a given $L$-layer MLP $f$ whose parameter is $\btheta=(\bW\lyr{1},\bW\lyr{2},\ldots,\bW\lyr{L})$ in \cref{eq:mlp} as
\[
% \label{eq:reparametrization}
&\bW\lyr{l} = \bP_{1:c}\lyr{l}\bV\lyr{l}\bQ_{1:d}\lyr{l},\quad\text{and}\quad\bb\lyr{l}=\bP_{1:d}\lyr{l}\ba\lyr{l},\quad\text{for }l=1,2,\ldots,L,\nonumber \\
&\bP_{1:c}\lyr{l} = \bP_{c}\lyr{l}\cdots\bP_2\lyr{l}\bP_1\lyr{l}\quad\text{and}\quad \bQ_{1:d}\lyr{l} = \bQ_1\lyr{l}\bQ_2\lyr{l}\cdots\bQ_{d}\lyr{l},
\]
where $\bV\lyr{l}\in\bbR^{n_l\times n_{l-1}}$ is a base weight matrix, $\bP_i\lyr{l}\in\bbR^{n_l \times n_l}$, $\bQ_i\lyr{l}\in\bbR^{n_{l-1} \times n_{l-1}}$ are the expanded matrices, and $e=c+d\geq 0$ is the number of the expanded matrices. We call this \emph{expanded parametrization} (EP), whereas $e=0$ denotes the standard parameterization (SP). Note that although $\bP_i\lyr{l}$ and $\bQ_i\lyr{l}$ are not necessary to be square matrices, their multiplication $\bP_{1:c}\lyr{l}$ and $\bQ_{1:d}\lyr{l}$ must be square matrices to maintain the dimension of $\bW$ when $\bV$ holds the dimension of $\bW$. Nonetheless, we set $\bP_i\lyr{l}$ and $\bQ_i\lyr{l}$ also square in order to save memory cost while preserving convergence stability of $\bP_{1:c}\lyr{l}$ and $\bQ_{1:d}\lyr{l}$, only guaranteed when the width of intermediate dimension of DLNN should be greater and equal to both input and output dimensions \citep{laurent2018deep,du2019width}.

The revised SGHMC due to the expanded parameters can be described as same as \cref{eq:sghmc}:
\[
\label{eq:qsghmc}
\btheta &\gets \btheta + \epsilon \bM^{-1} \bsr \nonumber\\
\bsr &\gets (1 - \epsilon \bC \bM^{-1}) \bsr - \epsilon \nabla_{\theta}\tilde{U}(\btheta) + \calN(0, 2(\bC - \hat{\bB}) \epsilon),\nonumber\\
&\quad\text{where}\quad\btheta = \left(\bP_{1}\lyr{l},\ldots,\bP_{c}\lyr{l},\bV\lyr{l},\bQ_{1}\lyr{1},\ldots,\bQ_{d}\lyr{l}\right)_{l=1}^L \nonumber\\
&\quad\text{and}\quad\br = \left(\bR_{1}\lyr{l},\ldots,\bR_{c}\lyr{l},\bS\lyr{l},\bT_{1}\lyr{1},\ldots,\bT_{d}\lyr{l}\right)_{l=1}^L.
\] In practice, we set the friction $\bC$ as a diagonal matrix whose diagonal elements are the same. However, when we reassemble the expanded parameter into $\bW$, the distribution of 

For simplicity of proofs, we treat SGLD instead of SGHMC in the comming theorems. The revised SGLD due to the expanded parameters can be described as
\[
\label{eq:qsgld}
\btheta &\gets \btheta - \epsilon \nabla_{\theta}\tilde{U}(\btheta) + \calN(0, 2\epsilon\bC)),\nonumber\\
&\quad\text{where}\quad\btheta = \left(\bP_{1}\lyr{l},\ldots,\bP_{c}\lyr{l},\bV\lyr{l},\bQ_{1}\lyr{1},\ldots,\bQ_{d}\lyr{l}\right)_{l=1}^L.
\]

\begin{thm}[Exploitation]
Consider SGLD with EP, $\bP_{1:c}\lyr{l}\bV\lyr{l}\bQ_{1:d}\lyr{l}$ as in \cref{eq:qsgld} and assume that the initialization of the parameters follows Theorem 1 in \citet{arora2018on} and the Gaussian noise of $\bP_i$ and $\bQ_j$ are zero for all $i\in[1,c]$ and $j\in[1,d]$. When the maximum singular value of EP across layers is bounded as
\[
\sup_l\sigma_\text{max}\left(\bP_{1:c}\lyr{l}\bV\lyr{l}\bQ_{1:d}\lyr{l}\right) \leq G,
\] and $\bbE\left[\norm{\partial U/\partial (\bP_{1:c}\lyr{l}\bV\lyr{l}\bQ_{1:d}\lyr{l})}_F\right]=h\lyr{l}\geq h$, then for any $\delta > 0$ and
\[
T \geq \frac{U_0-\delta}{\epsilon hL\cdot G^{2(c+d)/(c+d+1)}},
\] the potential energy at time step $T$ of SGLD with step size $\epsilon$, $\bbE[U_T]$ is always less than or equal to $\delta$, where $U_0$ denotes the potential energy at time step 0.
\end{thm}

\begin{proof}
    The proof consists of the calculating the upper bound of $\bbE[U_T]$. As in \citet{arora2019convergence}, we apply the gradient updates of the multiplied value $\bP\bV\bQ$ which differs from that of single matrix $\bV$ as described in the implicit acceleration of DLNN \citep{arora2018on}.

    When the gradient update of $\V{\bW}$ for an arbitary matrix $\bW$ is described as
    \[
    \V{\bW}(t)&=-\nabla_{\V{\bW}}\calF(\V{\bW}(t)), 
    \] where $\calF$ is an arbitrary function that determines the dynamics of $\bW(t)$, by Theorem 1 and Claim 1 in~\citet{arora2018on}, the dynamics of the multiplied parameters with vectorization $\bX=\left(\V{\bW_{1:e}\lyr{l}}\right)_{l=1}^L$ for $\bW_{1:e} = \bW_1\bW_2\cdots\bW_e$ is as follows:
    \[
    \dee\bX(t) = - P_{\bX(t)}\nabla\calF(\bX(t))\dee t,
    \] 
    % where $P_{\bX(t)}$ is a positive semi-definite matrix whose eigenvalues are greater than or equal to $\sigma_\text{min}(\bW_{1:e}(t))^{2(e-1)/e}$ when $\sigma_\text{min}$ denotes the minimum singular value.
    where $P_{\bX(t)}$ is a positive semi-definite matrix whose eigenvalues are less than or equal to $\sigma_\text{max}(\bW_{1:e}(t))^{2(e-1)/e}$ when $\sigma_\text{max}$ denotes the maximum singular value.
    
    In the SGLD setting, although the noise is added in contrast of Eq. 9 in \citet{arora2018on}, the expectation of the difference is still valid along the times steps $t$ as
    \[
    \bbE[\bW_{j+1}(t)\tr \bW_{j+1}(t)-\bW_j(t)\bW_j(t)\tr]=0,\quad\forall t\geq t_0,
    \] with a small variance. Thus, the same argument can be applied. Additionally, due to the only noise added in one of $\bW_i$, the noise of $\bW_{1:e}$ is still Gaussian so the diffusion dynamics of $\bW_{1:e}$ can be described as:
    \[
    \dee\bX(t) = - P_{\bX(t)}\nabla\tilde{U}(\bX(t))\dee t + B\dee W_t,
    \] where $\dee W_t$ is the Brownian motion and the $B$ is the noise scale. For the stochastic gradient assumption $\nabla\tilde{U} = \nabla U +\bss$ for a random variable $\bss$ such that $\bbE[\bss]= 0$,
    \[
    \dee\bX(t) = - P_{\bX(t)}(\nabla U(\bX(t))+\bss)\dee t + B\dee W_t,
    \]
    % The derivative of $U$ with respect to time can be decomposed using the chain rule: 
    % \[
    % \frac{\dee U(\bX(t))}{\dee t} &=\sum_{l=1}^L\left<\nabla U(\bX\lyr{l}(t)), \frac{\dee \bX\lyr{l}(t)}{\dee t}\right>\\
    % &=\sum_{l=1}^L\left<\nabla U(\bX\lyr{l}(t)), - P_{\bX\lyr{l}(t)}(\nabla U(\bX\lyr{l}(t))+\bss\lyr{l}) + B\lyr{l}\frac{\dee W_t}{\dee t}\right>\\
    % &\leq-\sum_{l=1}^L\sigma_\text{min}(\bW_{1:e}\lyr{l}(t))^{2(e-1)/e}\norm{\nabla U(\bX\lyr{l}(t))}^2 \\
    % &+ \sum_{l=1}^L\left<\nabla U (\bX\lyr{l}(t)),-P_{\bX\lyr{l}(t)}\bss\lyr{l}+B\lyr{l}\frac{\dee W_t}{\dee t}\right>
    % \] For the step size $\epsilon$, the potential difference between $t+1$ and $t$ steps is bounded by
    % \[
    % \lefteqn{U(\bX(t+1)) - U(\bX(t))}\nonumber\\
    % &\leq -\epsilon\sum_{l=1}^L\sigma_\text{min}(\bW_{1:e}\lyr{l}(t))^{2(e-1)/e}\norm{\nabla U(\bX\lyr{l}(t))}^2 + \sum_{l=1}^L\left<\nabla U(\bX\lyr{l}(t)),-\epsilon P_{\bX(t)}\bss\lyr{l}+\epsilon\bxi_t\right>,\\
    % &\leq -\epsilon\cdot g^{2(e-1)/e}\sum_{l=1}^L\norm{\nabla U(\bX\lyr{l}(t))}^2,\label{eq:bound1}
    % \] where $\bxi\sim\calN(0,I)$.

    From the local convexity of the potential energy $U$, the following holds:
    \[
    & U(\bX(t+1))-U(\bX(t)) \\
    & \geq \sum_{l=1}^L\left<\nabla U(\bX\lyr{l}(t)), \bX\lyr{l}(t+1)-\bX\lyr{l}(t)\right>\\
    &=\sum_{l=1}^L\left<\nabla U(\bX\lyr{l}(t)), -\epsilon P_{\bX\lyr{l}(t)}(\nabla U(\bX\lyr{l}(t)+\bss\lyr{l})+B\lyr{l}\bxi_t\right>\\
    &\geq -\epsilon \sum_{l=1}^L \sigma_\text{max}(\bW_{1:e}\lyr{l}(t))^{2(e-1)/e}\norm{\nabla U(\bX\lyr{l}(t)}^2+\sum_{l=1}^L\left<\nabla U(\bX\lyr{l}(t)),-\epsilon P_{\bX\lyr{l}(t)}\bss\lyr{l}+\epsilon B\lyr{l}\bxi_t)\right>\\
    &\geq -\epsilon G^{2(e-1)/e}\sum_{l=1}^L\norm{\nabla U(\bX\lyr{l}(t)}^2 +\sum_{l=1}^L\left<\nabla U(\bX\lyr{l}(t)),-\epsilon P_{\bX\lyr{l}(t)}\bss\lyr{l}+\epsilon B\lyr{l}\bxi_t)\right>. \label{eq:bound2}
    \] By taking expectation on the both sides,
    \[
    \bbE[U(\bX(t+1))]- \bbE[U(\bX(t))] &\leq -\epsilon G^{2(e-1)/e}\sum_{l=1}^L\bbE\left[\norm{\nabla U(\bX\lyr{l}(t)}^2\right].
    \] Taking summation from $t=0$ to $T-1$,
    \[
    \bbE[U(\bX(T))] &\leq \bbE[U(\bX(0))] -\epsilon G^{2(e-1)/e}\sum_{t=0}^{T-1}\sum_{l=1}^L\bbE\left[\norm{\nabla U(\bX\lyr{l}(t)}^2\right]\\
    &\leq U(\bX(0)) - \epsilon\cdot G^{2(e-1)/e}TLh,
    \]which concludes $\bbE[U(\bW(T))] \leq \delta$ if
    \[
    T \geq \frac{U(\bX(0))-\delta}{\epsilon hL\cdot G^{2(e-1)/e}}.
    \]
    
    % The summation from $t=0$ to $T-1$ on the both sides:
    % \[
    % U(\bX\lyr{l}(T)) &\leq U(\bX\lyr{l}(0)) - \epsilon\cdot\sum_{t=0}^{T-1}\sum_{l=1}^L\sigma_\text{min}(\bW_{1:e}\lyr{l}(t))^{2(e-1)/e}\norm{\nabla U(\bX\lyr{l}(t))}^2 \nonumber\\
    % &+\sum_{t=0}^{T-1}\sum_{l=1}^L\left<\nabla U(\bX\lyr{l}(t)),-\epsilon P_{\bX\lyr{l}(t)}\bss\lyr{l}+\epsilon\bxi\right>.
    % \] When $\sigma_\text{min}(\bW_{1:e}(t))\geq g$ and $\bbE[\norm{\nabla U(\bX(t))}]\leq h$, their expection for a fixed initial value $\bX(0)$ is bounded as
    % \[
    % \bbE[U(\bX(T))] &\leq U(\bX(0)) - \epsilon\cdot g^{2(e-1)/e}TLh \nonumber\\
    % &+\sum_{t=0}^{T-1}\bbE\sum_{l=1}^L\left[\left<\nabla U(\bX(t)),-\epsilon P_{\bX(t)}\bss+\epsilon\bxi\right>\right]\\
    % &= U(\bX(0)) - \epsilon\cdot g^{2(e-1)/e}TLh,
    % \] which concludes $\bbE[U(\bW(T))] \leq \delta$ if
    % \[
    % T \geq \frac{U(\bX(0))-\delta}{\epsilon hL\cdot g^{2(e-1)/e}}.
    % \]
\end{proof}

\begin{lem}[Dynamics of expanded parameters]
    For an arbitrary function $\calF$ whose parameter is $\bW_{1:e}=\bW_1\cdots\bW_e$ with its vectorization $\bX=\V{\bX_{1:e}}$, assume that the gradient update of each $\bW_i$ for $i\in[1,e]$ is defined as the following PDE:
    \[
    \dee\bW_i(t) = -\nabla_{\bW_i}\calF(\bW_1(t),\ldots,\bW_e(t))\dee t.
    \] Then, their multiplication $\bX$ satisfies the following dynamics:
    \[
    \lefteqn{\dee\bX(t) = -P_{\bX(t)}\nabla_{\bX}\calF(\bX(t))\dee t,}\\
    \text{where}\quad P_{\bX(t))} =& \bW_{2:e}\tr\bW_{2:e}\otimes I+\sum_{i=2}^{e-1} \left(\bW_{j+1:e}\tr\bW_{j+1:e}\otimes \bW_{1:j-1}\bW_{1:j-1}\tr\right)\\
    &+I\otimes\bW_{1:e-1}\bW_{1:e-1}\tr,
    \] where $\otimes$ is the Kronecker product and $P_{\bX(t)}$ is a positive semi-definite and symmetric matrix.
\end{lem}
\begin{proof}
    TBD
\end{proof}

\begin{thm}[Exploration]
    Let $f$ be an $H$-Lipschitz continuous function:
    \[
        \norm{f(\bX)-f(\bX')}_2\leq H\norm{\bX-\bX'}_2,
    \] and the expectations of norms of the gradients, stochastic gradient, and the Gaussian noise in~\cref{eq:qsgld} are bounded as
    \[
    \bbE\left[\norm{\nabla U(\bW\lyr{l}(t))}_2\right]&\leq h, \\
    \bbE\left[\norm{\nabla U(\bW\lyr{l}(t))-\nabla \tilde{U}(\bW\lyr{l}(t))}_2\right]&\leq s, \\
    \bbE[\norm{\bC}_2]&\leq C,
    \] and all the maximum singular value of each matrix be bounded as
    \[
        \sigma_\text{max}(\bP_i),\sigma_\text{max}(\bV),\sigma_\text{max}(\bQ_j) \leq m,\quad\forall i\in[1,c],\forall j\in[1,d].
    \]
    The upper bound of the output distance of samples between time steps of SGLD is bounded proportional to the depth $c+d+1$ as
    \[
    \norm{f(\bW(t))-f(\bW(t+1))}_2\leq \epsilon HL^{3/2}(c+d+1)^{1/2}\cdot m^{(c+d)/2}(h + s) + HC.
    \] i.e. the functional diversity between samples is tighter as the depth decreases.
\end{thm}
\begin{proof}
    For $\bX=\left(\V{\bW_{1:e}\lyr{l}}\right)_{l=1}^L$ such that $\bW_{1:e} = \bW_1\bW_2\cdots\bW_e$ and $\nabla \tilde{U}(\bX(t)) = \nabla U(\bX(t)) + \bss$ such that $\bbE[\norm{\bss}]=s$, the distance between the two adjacent time steps is bounded as
    \[
    \norm{\bX(t+1)-\bX(t)}_2 &\leq \epsilon\norm{-P_{\bX(t)}\nabla\tilde{U}(\bX(t)+B_t\bxi}_2 \\
    &\leq \epsilon\norm{P_{\bX(t)}}_2\norm{\nabla\tilde{U}(\bX(t))}_2 + \epsilon\norm{B_t\bxi}_2\\
    &\leq \epsilon\sqrt{\sum_{l=1}^L\sum_{j=1}^e\prod_{i\neq j}\sigma_\text{max}(\bW_i\lyr{l})}\left(\norm{\nabla U(\bX\lyr{l}(t))}_2 + \norm{\bss\lyr{l}}_2\right) + \epsilon\norm{B_t\bxi\lyr{l}}_2.
    \] Once we take the square root and expectation on both sides,
    \[
    \bbE\left[\norm{\bX(t+1)-\bX(t)}\right] &\leq\epsilon\bbE\left[\sqrt{\sum_{l=1}^L\sum_{j=1}^e\prod_{i\neq j}\sigma_\text{max}(\bW_i\lyr{l})}\left(\norm{\nabla U(\bX(t))}_2 + \norm{\bss}_2\right) + \norm{B_t\bxi}_2\right]\\
    &\leq\epsilon L^{1/2}e^{1/2}\cdot m^{(e-1)/2}(Lh + Ls) + HC
    \] By the $H$-Lipschitzness,
    \[
    \norm{f(\bX(t))-f(\bX(t+1))}_2\leq \epsilon HL^{3/2}e^{1/2}\cdot m^{(e-1)/2}(h + s) + C.
    \]
    
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Prior Distributions}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relationship to Riemannian Manifold LD and Preconditioned SGLD}
There is relationship only in langevin dynamics as a precondition matrix.

==> main/_deprecated_relatedwork.tex <==
\section{Related Work}
\label{sec:main:relatedwork}

\subsection{A Role of Symmetry in Bayesian Neural Networks}

\citet{entezari2022the} empirically demonstrates their conjecture that every two independent SGD solutions are linearly connected through a low loss path after we align the solution to be close to each other. This can be an evidence that every solutions can be located in the same basin through the alignment. We call this re-basin. The first re-basin method \citep{ainsworth2023git}, which puts two independent SGD solutions in a single basin through the permutation alignments, it suggested a surrogate method to align two solutions within polynomial time.

As an extension of linear mode connectivity, the distribution alignment technique \citep{rossi2023on} showed transport alignment of two variational distributions of BNN and their loss barriers were also reduced. It explains that BNN samples are also located nearby the other BNN samples, once accounting for the permutation.

Desire of approximating multi-modal distributions using a single variational distribution brought a design of permutation invariant variational distribution which estimates multi-modality raised from the permutation symmetry. \citet{gelberg2024variational} exhibited the variational inference via permutation invariant distribution improved the accruacy of BNNs.

Revisiting the Effects of Stochasticity for Hamiltonian Samplers \citep{franzese2022revisiting}

On the Symmetries of Deep Learning Models and their Internal Representations \citep{godfrey2022on}

REPAIR: REnormalizing Permuted Activations for Interpolation Repair \citep{jordan2023repair}

On the detrimental effect of invariances in the likelihood for variational inference \citep{kurle2022on}

Doubly Stochastic Variational Inference for Deep Gaussian Processes \citep{salimbeni2017doubly}

Geometry of the Loss Landscape in Overparameterized Neural Networks: Symmetries and Invariances \citep{simsek2021geometry}

Towards Efficient MCMC Sampling in Bayesian Neural Networks by Exploiting Symmetry (Extended Abstract) \citep{wiese2024towards}

Mechanistic Mode Connectivity

Re-Basin via Implicit Sinkhorn Differentiation

Proving Linear Mode Connectivity of Neural Networks via Optimal Transport

Deep Networks on Toroids: Removing Symmetries Reveals the Structure of Flat Regions in the Landscape Geometry

Symmetries, flat minima, and the conserved quantities of gradient flow

\subsection{Improving Exploration of SGMCMC}

cSGMCMC \citep{zhang2020cyclical} adopted an periodic step size scheduling in the SGMCMC. Each cycle consists of exploration stage (large step size) and sampling stage (small step size) in order, which take diversity from the large step size and good performance from the small step size.

Given multiple parallel chains, \citet{gallego2020stochastic} proposed a method to give a replusive force across the chains. it enforces them being distant each other so that the chains produces diverse samples.

Meta-Learning For Stochastic Gradient MCMC \citep{gong2019meta}

Learning to Explore for Stochastic Gradient MCMC \citep{kim2024learning}

Non-convex Learning via Replica Exchange Stochastic Gradient {MCMC} \citep{Deng2020nonconvex}

Structured Stochastic Gradient MCMC
